Confidential Inference via Ternary Model Partitioning

Today's cloud vendors are competing to provide various offerings to simplify and accelerate AI service deployment. However, cloud users always have concerns about the confidentiality of their runtime data, which are supposed to be processed on third-party's compute infrastructures. Information disclosure of user-supplied data may jeopardize users' privacy and breach increasingly stringent data protection regulations. In this paper, we systematically investigate the life cycles of inference inputs in deep learning image classification pipelines and understand how the information could be leaked. Based on the discovered insights, we develop a Ternary Model Partitioning mechanism and bring trusted execution environments to mitigate the identified information leakages. Our research prototype consists of two co-operative components: (1) Model Assessment Framework, a local model evaluation and partitioning tool that assists cloud users in deployment preparation; (2) Infenclave, an enclave-based model serving system for online confidential inference in the cloud. We have conducted comprehensive security and performance evaluation on three representative ImageNet-level deep learning models with different network depths and architectural complexity. Our results demonstrate the feasibility of launching confidential inference services in the cloud with maximized confidentiality guarantees and low performance costs.

==> Makefile <==
NAME=main

TARGET=$(NAME)
BIBTEX := bibtex
TGIF   := tgif
XFIG   := xfig
GNUPLOT:= gnuplot

SOURCES=$(wildcard *.tex) $(wildcard *.bib)

FIGS= $(wildcard figures/*)

all: $(TARGET).pdf
$(TARGET).pdf: Makefile  $(SOURCES) $(FIGS)
	pdflatex  $(TARGET).tex
	-bibtex --min-crossrefs=100    $(TARGET)
	pdflatex  $(TARGET).tex
	pdflatex  $(TARGET).tex

color: $(TARGET).pdf
	pdflatex $(TARGET).tex
	pdftops $(TARGET).pdf

$(TARGET).ps: $(TARGET).pdf
	pdflatex "\newcommand{\wantBW}{} \input{$(TARGET).tex}"
	pdftops $(TARGET).pdf

%.pdf : %.fig #Makefile
	fig2dev -L pdf -b 1 $< $@

%.eps : %.dia #Makefile
	dia --nosplash -e $@ $<

%.eps : %.obj
	TMPDIR=/tmp $(TGIF) -print -eps $<

%.pdf : %.eps #Makefile
	epstopdf $<

check:
	grep -nr "ﬂ\|ﬁ" .
	grep -nr "“" .
	grep -nr "’" .

clean:
	rm -f *.aux *.log *.out *.bbl *.blg *~ $(TARGET).dvi $(TARGET).pdf

==> background.tex <==
\section{Background}
\label{sec:background}

In this section, we give a brief overview of two technologies that are
closely related to our work: \emph{deep learning} and \emph{Intel SGX}.  
Deep learning is the key technology behind most
state-of-the-art artificial intelligence (AI) services. We leverage Intel SGX as the
Trusted Execution Environment (TEE) in \protoname{} to protect the
confidentiality of user input data in deep learning pipelines.

\nip{Deep Learning.}
Deep learning is an application of \emph{Artificial Neural Networks} and is in the family
of \emph{Representation Learning}. Deep learning methods can process
raw data directly and automatically discover the representations, with
no human interventions. It can learn complex functions by composing
multiple non-linear modules to transform representations from
low-level raw inputs to high-level abstractions.

The major component of any deep learning inference system is a DNN, which has
multiple hidden layers between the input and output layers.  Each
layer contains multiple neurons.  
Each connection between two neurons
in a DNN has an associated weight.  In supervised
learning, the weights are learned in the training stage by maximizing
the objective function of a neural network.  Generally, stochastic
gradient descent (SGD) with back-propagation is the most widely
used approach for learning the weights of neural networks.  

Mathematically, deep learning inference of a feedforward DNN can be defined as a representation function $F^*$ that maps an
input $\mathbf{x}$ to an output $\mathbf{y}$, i.e., $\mathbf{y} =
F^*(\mathbf{x};\mathbf{\theta})$. $\mathbf{\theta}$ represents parameters that are learned during model training. $F^*$ is composed of $n$ (assuming the network has
$n$ layers) sub-functions $F_i$, where $i \in [1, n]$. $F_i$ maps the
input $\mathbf{x}_i$ to the output $\mathbf{y}_i$ on layer $i$.  These
sub-functions are connected in a chain. Thus, $\mathbf{y} =
F^*(\mathbf{x};\mathbf{\theta}) = \mathit{F}_n
\mathit{F}_{n-1}...\mathit{F}_1(\mathbf{x})$.  
For a classification model, 
the final output $\mathbf{y}$ is a probability vector generated by the \emph{softmax} activation function. 
The top-k entries are extracted from $\mathbf{y}$ and are mapped with a set of user-defined class labels $\mathrm{L}$. 


\begin{comment}
Each neuron is a computational unit that receives an input vector
$\mathbf{x}$ from its connected neurons in the previous layer and a
bias signal $b$.  It first computes $z = \mathbf{w^T}\mathbf{x} + b =
\sum_{i=1}^{n} w_i x_i + b$, which is a weighted sum of its inputs.
After getting $z$, each neuron applies a non-linear activation
function $f$ and passes the result $f(z)$ to the connected neurons in
the next layer.  Popular activation functions include hyperbolic
tangent $f(z) = (e^{2z}-1)(e^{2z}+1)^{-1}$, sigmoid $f(z) =
(1+e^{-z})^{-1}$, and Rectified Linear Unit (ReLU) $f(z) = max(0, z)$.
If the purpose of the neural network is to classify data into a finite
number of classes, the activation function in the output (last) layer
usually is a softmax function $f(\mathbf{z})_j =
e^{z_j}\cdot(\sum_{n=1}^{N} e^{z_n})^{-1} \ \forall j \in [1,N]$.  The
output of a softmax function is a probability distribution over $N$
classes.






%A DNN is typically a feedforward neural network wherein connections between the neurons do not form a loop. 
%However, recurrent neural networks (RNNs), especially the long short-term memory (LSTM)~\cite{hochreiter1997long} networks,
%have loops in them and allow information to persist. 
%RNNs are widely used for processing dynamic temporal behavior. 
%In this work, we mainly focus on the feedforward deep neural network, but in principle, our approach can also be extended to support RNNs.

In addition, we briefly discuss Convolutional Neural Networks (ConvNets), which have achieved great
success in computer vision tasks, including detection, segmentation,
and recognition of objects in images and videos.  ConvNet is a class
of feedforward DNN that is designed for processing data in
multi-dimensional arrays.  Different from fully connected neural
networks, the neurons in each layer of a ConvNet are arranged in three
dimensions: \emph{width}, \emph{height}, and \emph{depth}.  Each neuron only connects to a
receptive field of a previous layer.  There are a few distinct types
of layers for ConvNets, including convolutional layers and pooling
layers.  The parameters of a convolutional layer consist of a set of
learnable filters.  Each filter computes a dot product between their
weights and a receptive field it connects to in the input volume, thus
producing a $2$-dimensional feature map.  A convolutional layer
usually uses Rectified Linear Unit (ReLU) as its activation function.  The output volume of a
convolutional layer is stacked feature maps along the \emph{depth} dimension.
The pooling layers perform non-linear down-sampling operations to
reduce the dimensionality of the feature maps.  The convolutional and
pooling layers in a ConvNet act as the feature extractors for the
input.  ConvNets use the same \emph{softmax} activation function for
classification, similar to a regular DNN.
\end{comment}

\nip{Intel SGX.}
SGX~\cite{mcKeen2013innovative} offers a non-hierarchical
protection model to support secure computation on untrusted remote
servers.  SGX includes a set of new instructions and memory protection
mechanisms added to the Intel CPU architecture.  A user-level
application can instantiate a hardware-protected container, denoted as
an \emph{enclave}.  An enclave resides in the application's address
space and guarantees confidentiality and integrity of the code and
data within it.  Privileged system software is not allowed to access or tamper with the code/data of an initialized enclave.  SGX also relies on remote attestation to establish trust with the remote party by verifying the authenticity of its underlying hardware and integrity of the initialized enclave. Thereafter, secrets for computation can be provisioned to the attested enclave via a secure channel.  

\begin{comment}
Here, we briefly discuss the life cycle of an SGX enclave.  The
detailed explanation and analysis of Intel SGX technology can be found
in Costan and Devadas~\cite{costan2016intel}.  SGX sets aside a memory
region, referred to as the \emph{Processor Reserved Memory} (PRM).
The CPU enforces memory access control of PRM to prevent any
out-of-enclave memory accesses.  \emph{Enclave Page Cache} (EPC)
stores the code and data of an enclave.  The state of all pages of the
EPC is maintained in the \emph{Enclave Page Cache Map} (EPCM).  A
user-mode application can ask system software to create
(\emph{ECREATE}) an enclave.  In the loading stage, the untrusted
system software requests CPU to copy the code and data (\emph{EADD})
into the EPC and assigns these memory pages to an enclave.  After all
memory pages are loaded, an enclave is initialized (\emph{EINIT})
and the cryptographic hash of the enclave content is finalized.
Before provisioning any secrets into an enclave, a client needs to
initiate remote attestation~\cite{anati2013innovative} to verify the
trustworthy level of hardware and the hash of the enclave's contents.
An application can only enter its enclave via pre-defined function
interfaces by executing a special instruction (\emph{EENTER}).  If
enclave code needs to invoke system calls, it should exit
(\emph{EEXIT}) the enclave because ring $0$ code is not allowed
inside an enclave.  To serve interrupts, page faults, or VM exits, the
CPU needs to perform \emph{Asynchronous Enclave Exits} (AEXs) to save
the CPU state and transfer control to a pre-specified instruction out
of the enclave.  In SGX2~\cite{mckeen2016intel}, Intel will support
dynamic memory management inside an enclave, which allows run-time
changes to enclave memory while maintaining the security properties.
\end{comment}

==> backup.tex <==
\begin{comment}

Our work builds on
insights by research efforts in understanding the internal principles
of DNNs\cite{zeiler2014visualizing,yosinski2015understanding,shwartz2017opening}.
As indicated in~\cite{zeiler2014visualizing}, for an image
classification DNN, the shallow layers respond more to low-level
photographic information (such as edges, corners, and contours, of the
original inputs). In contrast, deep layers represent more abstract and
class-specific information related to the final outputs.
Mapping these insights to the security domain, we argue that both ends of DNNs disclose information of the input data, while under different conditions. 
Low-level photographic information at shallow layers reveals precise contents of original inputs, which are straightforward for humans (as adversaries) to understand. 
Whereas, high-level abstract representations at deep
layers are not directly comprehensible by humans. 
But the information embedded within such representations can be deciphered via forward propagation if models' semantic class labels are left unprotected. 
Moreover, if adversaries have access to preceding model parameters, they can exploit input reconstruction~\cite{mahendran2015understanding,dosovitskiy2015inverting} or model interpretation~\cite{simonyan2013deep,springenberg2014striving,bach2015pixel,selvaraju2017grad} techniques via backward propagation to divulge more sensitive information of the original inputs. 

In this paper, we present \protoname{}, an enclave-based
model serving system to mitigate information exposure of input data in deep learning inference pipelines.  
We grant end users the privilege to partition each deep learning model into a \emph{FrontNet} and a \emph{BackNet} by exploiting the layered structure of neural networks.
To protect the confidentiality of user inputs, we propose to enclose both the \emph{FrontNet} (``entrance'') and the \emph{semantic class mapping} (``exit'') of a DNN into an isolated execution environment that is kept confidential and tamper-resistant to external computing stacks. 
In this work, we leverage Intel SGX to enforce isolated execution with memory access control and encryption protection. 
At the same time, we delegate \emph{BackNet} computation to execute out of enclaves. 
Therefore, we can still benefit from the performance
improvements if cloud machines are equipped with AI-accelerated hardware.
By tightly confining both ends of a DNN within a secure enclave, we can eliminate the attacker's possibility of inferring inputs' attributions or reconstructing inputs, which rely on white-box access to model parameters for forward/backward propagation. 

Another key challenge of our approach is to determine the optimal
model-specific partitioning layers that balance the confidentiality
and performance requirements.  
We need to guarantee that the outputs of an enclaved \emph{FrontNet} should no longer reflect the semantic information of their corresponding inputs.  
We develop an offline \emph{neural network assessment framework} to
measure the similarity between inputs and their outputs of \emph{FrontNets}
with different numbers of layers.
End users can use this tool to automate the process of finding
optimal partitioning layers for their proprietary models.  
We have conducted partitioning experiments on three
ImageNet-level DNNs, i.e., \emph{Darknet Reference Model} (17
layers)\cite{reference}, \emph{Extraction Model} (28
layers)\cite{extraction}, and \emph{DenseNet Model} (306
layers)\cite{huang2017densely}, with different network depths and
architectural complexity.
Our comprehensive partitioning analysis and workload measurement can be used as a
guideline for end users to determine their own principle for
partitioning DNNs, thus to achieve maximized security and performance
guarantees.

\end{comment}


We consider that the adversaries might have some background knowledge
$B$ for reconstructing the sensitive original input $\mathbf{x}$.  The
background knowledge includes: (1) the domain knowledge of user
inputs, e.g., input file types and natural image
priors\cite{mahendran2015understanding}; (2) the knowledge on the
distribution of all bits of $\mathbf{x}$, which can be described by a
probability matrix $P = \{\ldots, p_{ij}, \ldots\}$, where $p_{ij}$ is
the probability that the $i$-th bit of $\mathbf{x}$ takes the value
$j$, $1\leq i \leq |\mathbf{x}|$ and $j\in \Omega$, $\Omega$ is the
encoding alphabet, and $\forall i, \sum_{j} p_{ij} = 1$.

Adversaries aim to reveal the sensitive information from inference input $\mathbf{x}$: given
an $\mathrm{IR} \in\mathbb{IR}$ of $\mathbf{x}$ and the background
knowledge $\mathrm{B}$, adversaries can devise an attack strategy
$\mathtt{S}$ to return $\tilde{\mathbf{x}}$, the reconstructed version of $\mathbf{x}$.  The attack strategy $\mathtt{S}$ may include (1) reconstructing inputs from IRs by approximating the inverse models; (2) interpreting IRs to reveal attribution information from inputs; (3)
inspecting IRs by projecting them to pixel space.  The \emph{FrontNet}'s representation function $\Phi(\cdot)$ is
considered to violate the $\epsilon$-\emph{confidentiality} for
$\mathbf{x}$, if there exists an attack strategy $\mathrm{S}$,
background knowledge $\mathrm{B}$ and intermediate representation
$\mathrm{IR}$,
\begin{equation}
\quad \frac{\mathsf{dist}[\mathbf{x}, \tilde{\mathbf{x}} | \tilde{\mathbf{x}}\leftarrow\mathrm{S} (\mathrm{B} ,\mathrm{IR})]}{\mathsf{dist}[\mathbf{x}, \tilde{\mathbf{x}} | \tilde{\mathbf{x}} \leftarrow \mathrm{S}(\mathrm{B})]} \leq \epsilon, \label{eq:privacy_bound}
\end{equation}

\noindent
where $\epsilon$ is the parameter to bound the distances between
$\mathbf{x}$ and $\tilde{\mathbf{x}}$ before and after observing
$\mathrm{IR}$ and $\epsilon \in [0, 1]$.  The $\mathsf{dist}$ measures
the distance between an original input $\mathbf{x}$ and a
reconstructed input $\tilde{\mathbf{x}}$.  Specifically,
$\mathsf{dist}[\mathbf{x}, \tilde{\mathbf{x}} | \tilde{\mathbf{x}}
  \leftarrow \mathrm{S}(\mathrm{B})]$ considers that
$\tilde{\mathbf{x}}$ is reconstructed only based on adversaries'
background knowledge $\mathrm{B}$.  Whereas in
$\mathsf{dist}[\mathbf{x}, \tilde{\mathbf{x}} | \tilde{\mathbf{x}}
  \leftarrow \mathrm{S}(\mathrm{B} ,\mathrm{IR})]$,
$\tilde{\mathbf{x}}$ is reconstructed based on both the adversaries'
background knowledge $B$ and the observed $\mathrm{IR}$.
Eq.~(\ref{eq:privacy_bound}) says that the true inference input
$\mathbf{x}$ is breached if adversaries can significantly reduce the
distance between $\tilde{\mathbf{x}}$ and $\mathbf{x}$ after obtaining
the $\mathrm{IR}$ of $\mathbf{x}$.


\subsection{Model Partitioning Strategy}
\label{ssec:partition}


To effectively protect the confidentiality of user inference data by enabling partitioned deep learning inference, one key research challenge is to determine the optimal model-specific partitioning layers for different DNNs. 
The general principle is that the outputs of an in-enclave \emph{FrontNet} should not be similar to its inputs. 
After satisfying this security condition, we can assign as many layers as possible to the \emph{BackNet}, which is supposed to run out of the enclave.  

Based on our threat model, we assume that the adversaries are able to retrieve the IR data of the layers located out of SGX enclaves, even though the IRs may only reside in the computer memory. 
Therefore, it is crucial to investigate whether this adversary can infer the contents of the original inputs by viewing the IRs. 
In DNNs, IRs are organized in the forms of stacked feature maps. 
Thus we project all feature maps back to the pixel space and save them as IR images. 
For example, if the output of one layer is a $112 \times 112 \times 64$ tensor, we can generate 64 IR images (112 in width and 112 in height). 

One partitioning method is to let human subjects view all IR images and pick the ones that reveal the original input $\mathbf{x}$'s information. 
However, this task is tedious and error-prone for human beings considering the quantity of IR images they need to inspect and is also difficult to quantify the distance between $\mathbf{x}$ and IRs.  
Instead, we replace human subjects with another DNN (by exploiting deep learning model's visual recognition capability) to automatically assess all IR images and identify the ones revealing most input information at each layer. 
This approach is based on the insight that if an IR image retains similar contents as the input image, it will be classified into similar categories.  
By measuring the similarity of classification results, we can deduce whether a specific IR image is visually similar to its original input. 
End users can leverage the assessment results to determine the optimal partitioning layers for different neural network architectures.   

\subsubsection{Neural Network Assessment Framework}
\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{./figures/dnnvalidation.pdf}
\caption{The Architecture of the \emph{Neural Network Assessment Framework}}
\label{fig:dnnvalidation}
\end{figure}

In Figure~\ref{fig:dnnvalidation}, we present the dual-neural-network architecture of our \emph{neural network assessment framework}. 
We submit an input $\mathbf{x}$ to the IR Generation Network (\emph{IRGenNet}) and generate $\mathrm{IR_i} \ i \in \left[1,n\right]$. 
We place the DL model that is to be deployed in the public cloud as the \emph{IRGenNet} to generate IRs.
Each $\mathrm{IR_i}$ contains multiple feature maps after passing Layer $i$ ($L_i$). 
Then we project feature maps to IR images and submit them to the IR Validation Network (\emph{IRValNet}), which acts as an oracle to inspect the IR images. 
The \emph{IRValNet} can have different model architecture/weights from the \emph{IRGenNet}.
We use the \emph{DenseNet Model}\cite{huang2017densely}, which is known for its high accuracy in image classification, as the oracle \emph{IRValNet} to verify the information exposure. 
The output of the \emph{IRValNet} is a $N$-dimensional ($N$ is the number of classes) probability vector with class scores.
We use the Kullback-Leibler (KL) divergence to measure the similarity of classification results.
At each Layer $i$, we select the IR image having the minimum KL divergence ($D_{KL}$) with the input $\mathbf{x}$ to quantitatively measure the $\mathsf{dist}[\mathbf{x}, \mathrm{IR_i}]$: $\forall j \in [1, \mathrm{d(L_i)}]$, where $\mathrm{d(L_i)}$ is the depth of the output tensor of Layer $i$.
\begin{equation}
\begin{split}
\mathsf{dist}[\mathbf{x}, \mathrm{IR_i}] &= \emph{min}_j(D_{KL}(F^*(\mathbf{x}, \theta)\ ||\ F^*(\mathrm{IR_{ij}}, \theta))) \\
&= \emph{min}_j(\sum^{N}_{k=1} F^*(\mathbf{x}, \theta)_{[k]} \log \frac{F^*(\mathbf{x}, \theta)_{[k]}}{F^*(\mathrm{IR_{ij}}, \theta)_{[k]}}),
\end{split}
\label{eq:kl}
\end{equation}

where $F^*(\cdot, \theta)$ is the representation function of \emph{IRValNet}.  
To determine the optimal partitioning layer for each neural network, we also compute $D_{KL}(F^*(\mathbf{x}, \theta) \ ||\ \mu)$ where $\mu \sim \mathtt{U}\,\{1, N\}$, the discrete uniform distribution of the probability vector, and $N$ is the number of classes. This represents that adversaries have no prior knowledge of
$\mathbf{x}$ before obtaining IRs and consider that $\mathbf{x}$ will be classified to any class with equal chance. Based on Eq.~(\ref{eq:privacy_bound}), we can compute
$\delta_i = \frac{\mathsf{dist}[\mathbf{x}, \mathrm{IR_i}]}{D_{KL}(F^*(\mathbf{x}, \theta)\ ||\ \mu)}$
and compare $\delta_i$ with the user-specified $\epsilon$ bound. For example, if the user chooses $\epsilon = 1$ to avoid violating $\epsilon$-\emph{confidentiality}, it is safe to partition at Layer $i$ only if $\delta_i > \epsilon = 1$. 
%It is worth noting that comparison with the uniform distribution with $\epsilon = 1$ is a very tight bound for the information exposure. 
%In the real-world scenario, we grant end users the freedom to determine their specific $\epsilon$ bound to satisfy their confidentiality requirements and balance between security and efficiency.
In Section~\ref{ssec:partanalysis}, we leverage the \emph{neural network assessment framework} to analyze three representative deep learning models and determine their corresponding optimal \emph{FrontNet}/\emph{BackNet} partitioning.  


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\begin{comment}
\subsection{SGX Side Channel Attacks.}
\label{sec:sgxsidechannel}
Since the inception of SGX as a TEE with a strong threat model, i.e., to guarantee confidentiality and integrity of computation upon untrusted or adversarial system software, we have observed research studies on a spectrum of side channels to extract sensitive information from enclave execution. 
These side channels include page faults\cite{xu2015controlled}, high resolution timers\cite{hahnel2017high}, branch history\cite{lee2017inferring}, memory management\cite{wang2017leaky}, CPU cache\cite{hahnel2017high,brasser2017software,gotzfried2017cache}, etc. In these case studies, side channel attacks have been explored and applied to extract and further to infer sensitive information from various SGX-protected applications.

We have not observed any SGX side channel attacks to recover inputs of deep neural networks by now and we consider that such tasks are exceedingly difficult due to the special computation model of neural networks. For existing SGX side channel attacks, the attackers need to eavesdrop the side channel signals that leak the control transfer information. However, the memory access patterns of deep neural network computation do not depend on the input data. Thus it is impossible to recover input instance with the leaked side channel information. In addition, in our design for \protoname{}, the \emph{FrontNet} of the model is encrypted. This makes the prerequisites (availability of source code or binaries of target programs) for SGX side channel attacks unsatisfied.

However, through side channels, it is still possible to recover model hyperparameters, e.g., filter strides, activation function types, or the size of the inputs, which are pre-defined by deep learning model builders.  
Furthermore, if a deep learning image classification service needs to handle JPEG files as inputs, the file preprocessing procedure, i.e., the extraction of the pixel content of the images, may invoke some JPEG library functions, which have been demonstrated to be potentially vulnerable to side-channel attacks\cite{xu2015controlled,hahnel2017high}.

The side-channel attacks mentioned above can be addressed by enclave code developers to avoid secret-dependent program logic.  
However, recent security disclosures, e.g., \emph{Foreshadow}\cite{vanbulck2018foreshadow} and \emph{SGXPectre}\cite{chen2018sgxpectre}, demonstrate that speculative execution in micro-architectural implementation can potentially leak in-enclave secret data. 
Such vulnerabilities require firmware/hardware-level updates and can only be addressed by Intel. We expect that \protoname{} should be running on a trusted processor package with these vulnerabilities fixed.    
\end{comment}

\begin{comment}
\subsection{Applicable Deep Learning Models.}
\label{sec:autoencoder}
In addition to the widely deployed deep learning models used for classification tasks, 
there also exist some special \emph{information-preserving} neural networks designed for specific machine learning purposes. 
One representative case is the AutoEncoder~\cite{hinton2006reducing}, which is used for efficient encoding, dimension reduction, and learning generative models. 
AutoEncoder networks are trained to minimize the reconstruction errors between inputs and outputs.
Thus, an AutoEncoder's outputs may contain similar sensitive information as its inputs.
Our system can be naturally extended to support confidentiality protection of AutoEncoder's inputs.
We need to partition each AutoEncoder neural network into three sub-models, i.e., \emph{FrontNet}, \emph{MiddleNet}, and \emph{BackNet}. 
Then we can enclose both the \emph{FrontNet} and the \emph{BackNet} into an isolated enclave, as both ends of the AutoEncoder may generate IRs similar to the original inputs. 
End users can use our \emph{Neural Network Assessment Framework} to determine the number of layers assigned respectively for the \emph{FrontNet} and the \emph{BackNet}. 
\end{comment}



==> motivation.tex <==
\section{Information Disclosure Analysis}
\label{sec:motivation}
\begin{figure*}[!ht]
\centering
\includegraphics[width=1\textwidth]{./figures/privacy.pdf}
\caption{The Information Disclosure of Input Data in a Deep Learning Inference Pipeline}
\label{fig:privacy}
\end{figure*}
We investigate the life cycles of input data instances in the deep learning image classification pipelines and intend to identify the potential places where information might leak. 
We give a motivating example in
Figure~\ref{fig:privacy} to empirically demonstrate such information
disclosure.  We feed this picture\footnote{Image source: \url{https://www.tesla.com/software}} into a 1000-class image
classification system. This classifier is powered by a convolutional neural network (ConvNet) trained on the ImageNet dataset.  
The output of the system is the top-5 prediction class scores of the picture. 

We first present the potential information disclosure that may occur in the deep learning inference pipelines.
Thereafter, we describe the security principles our system needs to achieve to mitigate each type of information disclosure respectively. 


\subsection{Information Disclosure in Inputs}
If the inputs are fed into a DL inference system without being properly encrypted, adversaries may directly learn sensitive and private information.  

For this specific example, adversaries can infer the location of this car based on the map and GPS information \ovalbox{\footnotesize 1}.
The night mode of the map uncovers the approximate time when this picture was taken.  
In addition, the steering wheel emblem \ovalbox{\footnotesize 2}
reveals the car model and the digital speedometer \ovalbox{\footnotesize 3} shows the speed.
Adversaries can also obtain more personal information about the driver from the
album list \ovalbox{\footnotesize 4} of the media player and the car settings \ovalbox{\footnotesize 5} on the touchscreen.  
Furthermore, if the picture's EXIF meta-data are not carefully
eliminated, adversaries may also retrieve the GPS coordinates, the original
date and time when the picture was taken, the device type, and all
camera configurations from the EXIF, which may disclose more private
information about the user. 

Therefore, our system need to guarantee that the original inputs shall not be exposed without proper protection on cloud machines. We define the first security principle to prevent information disclosures in the original inputs.

\begin{tcolorbox}[enhanced,attach boxed title to top center={yshift=-3mm,yshifttext=-1mm},
  colback=gray!5!white,colframe=black!75!black,colbacktitle=gray!80!black,
  title=Security Principle I,fonttitle=\bfseries,
  boxed title style={size=small,colframe=black!50!black} ]
Confidentiality protection should be enforced to prevent adversaries from directly inspecting the contents of the inputs.
\end{tcolorbox}

\subsection{Information Disclosure in IRs}
A deep learning inference procedure extracts feature representations layer by layer.  
The process can be formulated as a composite transformation function that maps raw inputs to outputs.  
Each hidden layer performs its own transformation as a sub-function and generates an intermediate representation (IR) as an output.  
A transformation at each hidden layer helps converge the IRs towards the final outputs.
Based on the research efforts in understanding the internal mechanisms
of DNNs\cite{zeiler2014visualizing,yosinski2015understanding,shwartz2017opening}, 
for an image classification DNN, the shallow layers respond more to low-level
photographic information (such as edges, corners, and contours, of the
original inputs). In contrast, deep layers represent more abstract and
class-specific information related to the final outputs.

Mapping these insights to the security domain, IRs computed out of shallow and deep layers may disclose different input information depending on adversaries' capability. We summarize three types of information disclosure in IRs as follows:


\paragraph{Explicit Disclosure via Projected IRs}
IRs computed out of shallow layers still bestow low-level photographic information of the original inputs. Thus, it is straightforward for humans, acting as adversaries, to understand the IRs by projecting them to pixel space. 
For example, in Figure~\ref{fig:privacy},
by examining the contents of the IR images out of shallow layers, adversaries are able to collect similar amount of information (though with a certain level of information loss) if compared with inspecting the original input directly. We consider that such IRs at shallow layers explicitly disclose the visual information of the original inputs. Therefore, we derive the second security principle intending to prevent the explicit information disclosure in IRs. 

\begin{tcolorbox}[enhanced,attach boxed title to top center={yshift=-3mm,yshifttext=-1mm},
  colback=gray!5!white,colframe=black!75!black,colbacktitle=gray!80!black,
  title=Security Principle II,fonttitle=\bfseries,
  boxed title style={size=small,colframe=black!50!black} ]
Confidentiality protection should be enforced to prevent adversaries from inspecting the IRs that are content-wise similar to the original inputs.
\end{tcolorbox}


By progressing towards deeper layers, the projected IR images in pixel space are not \emph{directly} comprehensible. 
The information of the original inputs is transformed into high-level features and is encoded via preceding layers as an encoder function. 
However, the information is still preserved within IRs and is crucial for final classification decisions. 
If adversaries can obtain both \emph{IRs} and \emph{the preceding model parameters}, they can still implicitly divulge sensitive information of the original inputs by exploiting \emph{input reconstruction}~\cite{mahendran2015understanding,dosovitskiy2015inverting} or \emph{model interpretation}~\cite{simonyan2013deep,springenberg2014striving,bach2015pixel,selvaraju2017grad} techniques. 
We analyze both types of implicit disclosures respectively in detail as follows. 

\paragraph{Implicit Disclosure via Input Reconstruction}
\label{para:reconstruct}
We consider that adversaries intend to reconstruct the original inputs from the IRs. 
The general input reconstruction problem in deep neural networks can be defined as follows: the representation function at layer $i$ of a given DNN is $\Phi : \mathbb{R}^{w \times h \times c} \mapsto \mathbb{R}^d$, wherein $\mathbb{R}^{w \times h \times c}$  is the input space of a specific
DNN and $\mathbb{R}^d$ is the output space for the IRs. 
This process transforms the input $\mathbf{x}$ to $\Phi(\mathbf{x};
\mathbf{\theta}_{\Phi})$ and 
$\mathbf{\theta}_{\Phi}$ represents the model parameters of the first $i$ layers.
Given an $\mathrm{IR} = \Phi(\mathbf{x};
\mathbf{\theta}_{\Phi})$, adversaries tend to compute an approximated inverse function $\phi^{-1}$ to generate $\tilde{\mathbf{x}} = \phi^{-1}(\mathrm{IR})$ that minimizes the distance between $\mathbf{x}$ and $\tilde{\mathbf{x}}$. In practice, in order to derive $\phi^{-1}$, adversaries need to have either \emph{white-box}~\cite{mahendran2015understanding} or \emph{black-box}~\cite{dosovitskiy2015inverting} access to $\Phi$. \emph{White-box} access means that adversaries need to retrieve the model parameters $\mathbf{\theta}_{\Phi}$, while \emph{black-box} access means that adversaries need to query $\Phi$ and generate input-IR pairs. The pairs can be further utilized to approximate a surrogate inverse model $\phi^{-1}$. 

\paragraph{Implicit Disclosure via Model Interpretation}
Instead of reconstructing the original inputs, adversaries can also exploit the model interpretation techniques, e.g., Deconv~\cite{zeiler2014visualizing}, Guided Backpropagation~\cite{springenberg2014striving}, LRP~\cite{bach2015pixel}, CAM~\cite{zhou2016learning}, Grad-CAM~\cite{selvaraju2017grad}, to interpret the numerical values in IRs. 
The attack strategy is to connect features in IRs to specific input attributions.   
Once such feature attribution or interpretation is established, it can be generalized to infer sensitive properties for future inputs. 
For example, some specific neurons may only be activated by a special attribution in the input, e.g., the \emph{steering wheel} in Figure~\ref{fig:privacy}. If adversaries can confirm the connection between a \emph{steering wheel} (as an input attribution) with a set of activated neurons, they can infer whether future inputs have the \emph{steering wheel} attribution by only checking the feature map activation.  

Similar as the information disclosure via input reconstruction, interpreting the numerical values in IRs also requires \emph{white-box} access to the model parameters. Thus, we can derive the third security principle for both cases above. 

\begin{tcolorbox}[enhanced,attach boxed title to top center={yshift=-3mm,yshifttext=-1mm},
  colback=gray!5!white,colframe=black!75!black,colbacktitle=gray!80!black,
  title=Security Principle III,fonttitle=\bfseries,
  boxed title style={size=small,colframe=black!50!black} ]
  Model parameters that generate IRs should be properly protected from both white-box access and black-box query to prevent input reconstruction and model interpretation.
\end{tcolorbox}

\subsection{Information Disclosure in Semantic Class Mapping}
The last place that might disclose the input information is at the exit of the deep learning inference pipeline. 
The semantic class mapping of a classifier leaks categorical information of the input. 
From the top-5 prediction results (\emph{racer}, \emph{beach wagon},
\emph{limousine}, \emph{sports car}, or \emph{cab}, with
different probability scores), we can clearly infer that this picture is highly related to a vehicle, without observing the original input.  
Therefore, IRs can be deciphered via forward propagation if a model's semantic class labels are left unprotected. 
To prevent the information disclosure at semantic mapping, we derive the fourth security principle.

\begin{tcolorbox}[enhanced,attach boxed title to top center={yshift=-3mm,yshifttext=-1mm},
  colback=gray!5!white,colframe=black!75!black,colbacktitle=gray!80!black,
  title=Security Principle IV,fonttitle=\bfseries,
  boxed title style={size=small,colframe=black!50!black} ]
  Confidentiality protection should be enforced for the models' semantic labels and the label mapping process.
\end{tcolorbox}


In summary, information disclosure of user input data might happen at multiple stages in a deep learning inference pipeline, such as data entrance, feature extraction, and semantic class mapping. The design of our system should take all the derived security principles into consideration to mitigate potential information leakages. 



==> problem.tex <==
\section{Problem Definition}
\label{sec:problem}

Based on the layered structure of deep neural networks, we partition
each network into two independent subnet models, i.e., a
\emph{FrontNet} and a \emph{BackNet}.  

Mathematically, a deep neural
network can be defined as a function $\mathit{F^*}$ that maps an
input $\mathbf{x}$ to an output $\mathbf{y}$, i.e., $\mathbf{y} =
\mathit{F^*}(\mathbf{x};\mathbf{\theta})$. $\mathbf{\theta}$ represents parameters that are learned during model training. $\mathit{F^*}$ is composed of $n$ (assuming the network has
$n$ layers) sub-functions $F_i$, where $i \in [1, n]$. $F_i$ maps the
input $\mathbf{x}_i$ to the output $\mathbf{y}_i$ on Layer $i$.  These
sub-functions are connected in a chain. Thus, $\mathbf{y} =
\mathit{F^*}(\mathbf{x};\mathbf{\theta}) = \mathit{F}_n
\mathit{F}_{n-1}...\mathit{F}_1(\mathbf{x})$.  


After partitioning the
neural network at the $m$-th layer where $m \in [1, n)$, the function
for \emph{FrontNet} can be represented as $\Phi : \mathbb{X} \mapsto
\mathbb{IR}$, wherein $\mathbb{X}$ is the input space of a specific
DNN and $\mathbb{IR}$ is the output space for the intermediate
representations. $\mathrm{IR} = \Phi(\mathbf{x};
\mathbf{\theta}_{\Phi})= \mathit{F}_m
\mathit{F}_{m-1}...\mathit{F}_1(\mathbf{x})$ and its output
$\mathrm{IR}$ is an intermediate representation computed out of a
\emph{FrontNet}.  The function $\lambda$ for a \emph{BackNet} is
$\mathrm{O} = \lambda(\mathrm{IR}; \mathbf{\theta}_\lambda) = \mathit{F}_n
\mathit{F}_{n-1}...\mathit{F}_{m+1}(\mathrm{IR})$, in which
$\mathrm{IR}$ is the input. The final output $\mathrm{O}$ of a \emph{BackNet} is a probability vector. The top-k entries are extracted from $\mathrm{O}$ and are mapped with a set of user-defined class labels $\mathrm{L}$. We designate this semantic class mapping procedure as $\eta(\mathrm{top}_k(\mathrm{O}); \mathrm{L})$.   

We consider that the adversaries might have some background knowledge
$B$ for reconstructing the sensitive original input $\mathbf{x}$.  The
background knowledge includes: (1) the domain knowledge of user
inputs, e.g., input file types and natural image
priors\cite{mahendran2015understanding}; (2) the knowledge on the
distribution of all bits of $\mathbf{x}$, which can be described by a
probability matrix $P = \{\ldots, p_{ij}, \ldots\}$, where $p_{ij}$ is
the probability that the $i$-th bit of $\mathbf{x}$ takes the value
$j$, $1\leq i \leq |\mathbf{x}|$ and $j\in \Omega$, $\Omega$ is the
encoding alphabet, and $\forall i, \sum_{j} p_{ij} = 1$.

Adversaries aim to reveal the sensitive information from inference input $\mathbf{x}$: given
an $\mathrm{IR} \in\mathbb{IR}$ of $\mathbf{x}$ and the background
knowledge $\mathrm{B}$, adversaries can devise an attack strategy
$\mathtt{S}$ to return $\tilde{\mathbf{x}}$, the reconstructed version of $\mathbf{x}$.  The attack strategy $\mathtt{S}$ may include (1) reconstructing inputs from IRs by approximating the inverse models; (2) interpreting IRs to reveal attribution information from inputs; (3)
inspecting IRs by projecting them to pixel space.  The \emph{FrontNet}'s representation function $\Phi(\cdot)$ is
considered to violate the $\epsilon$-\emph{confidentiality} for
$\mathbf{x}$, if there exists an attack strategy $\mathrm{S}$,
background knowledge $\mathrm{B}$ and intermediate representation
$\mathrm{IR}$,
\begin{equation}
\quad \frac{\mathsf{dist}[\mathbf{x}, \tilde{\mathbf{x}} | \tilde{\mathbf{x}}\leftarrow\mathrm{S} (\mathrm{B} ,\mathrm{IR})]}{\mathsf{dist}[\mathbf{x}, \tilde{\mathbf{x}} | \tilde{\mathbf{x}} \leftarrow \mathrm{S}(\mathrm{B})]} \leq \epsilon, \label{eq:privacy_bound}
\end{equation}

\noindent
where $\epsilon$ is the parameter to bound the distances between
$\mathbf{x}$ and $\tilde{\mathbf{x}}$ before and after observing
$\mathrm{IR}$ and $\epsilon \in [0, 1]$.  The $\mathsf{dist}$ measures
the distance between an original input $\mathbf{x}$ and a
reconstructed input $\tilde{\mathbf{x}}$.  Specifically,
$\mathsf{dist}[\mathbf{x}, \tilde{\mathbf{x}} | \tilde{\mathbf{x}}
  \leftarrow \mathrm{S}(\mathrm{B})]$ considers that
$\tilde{\mathbf{x}}$ is reconstructed only based on adversaries'
background knowledge $\mathrm{B}$.  Whereas in
$\mathsf{dist}[\mathbf{x}, \tilde{\mathbf{x}} | \tilde{\mathbf{x}}
  \leftarrow \mathrm{S}(\mathrm{B} ,\mathrm{IR})]$,
$\tilde{\mathbf{x}}$ is reconstructed based on both the adversaries'
background knowledge $B$ and the observed $\mathrm{IR}$.
Eq.~(\ref{eq:privacy_bound}) says that the true inference input
$\mathbf{x}$ is breached if adversaries can significantly reduce the
distance between $\tilde{\mathbf{x}}$ and $\mathbf{x}$ after obtaining
the $\mathrm{IR}$ of $\mathbf{x}$.

